Learning to Parse Wireframes in Images of Man-Made Environments

In this paper, we propose a learning-based approach to the task of automatically extracting a "wireframe" representation for images of cluttered man-made environments. The wireframe (see Fig. 1) contains all salient straight lines and their junctions of the scene that encode efficiently and accurately large-scale geometry and object shapes. To this end, we have built a very large new dataset of over 5,000 images with wireframes thoroughly labelled by humans. We have proposed two convolutional neural networks that are suitable for extracting junctions and lines with large spatial support, respectively. The networks trained on our dataset have achieved significantly better performance than state-of-the-art methods for junction detection and line segment detection, respectively. We have conducted extensive experiments to evaluate quantitatively and qualitatively the wireframes obtained by our method, and have convincingly shown that effectively and efficiently parsing wireframes for images of man-made environments is a feasible goal within reach. Such wireframes could benefit many important visual tasks such as feature correspondence, 3D reconstruction, vision-based mapping, localization, and navigation. The data and source code are available at https://github.com/huangkuns/wireframe.

==> 4model-kun.tex <==
% !TEX root = cvpr18-parsing.tex

\section{Wireframe Detection Method}

Recently, deep convolutional neural networks (CNNs) such as~\cite{SermanetEZMFL13, RenHGS15, RedmonF16} have shown impressive performance in object detection tasks. Utilizing the dataset we have, we here design new, end-to-end trainable CNNs for detecting junctions and lines, respectively, and then merge them into a complete wireframe. Fig.~\ref{fig:system} shows the overall architecture of our proposed networks and method. Note that we choose different network architectures for junctions and lines due to the nature of their geometric properties, which we will elaborate below.

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.95\textwidth]{plot/net.pdf}
	\caption{Architecture of the overall system. {\bf Top:} junction detection network. {\bf Bottom:} line detection network.\vspace{-5mm}}
	\label{fig:system}
\end{figure*}

\subsection{Junction Detection}

\subsubsection{Design Rationale} \vspace{-2mm}

\begin{figure}[t]
\centering
\includegraphics[width=0.35\textwidth]{plot/junction-def.pdf}\vspace{-1mm}
\caption{Representation of a junction with three branches. \vspace{-5mm}}
\label{fig:model}
\end{figure}

Our design of the network architecture is guided by several important observations about junctions.

\noindent{\bf Fully convolutional network for global detection.} As we mentioned before, \emph{local} junction detection is a difficult task, which often leads to spurious detections. Therefore, it is important to enable the network to reason globally when making predictions. This motivates us to choose a \emph{fully convolutional network} (FCN), following its recent success in object detection~\cite{RedmonF16}. Unlike other popular object detection techniques that are based on sliding windows~\cite{SermanetEZMFL13} or region proposals~\cite{RenHGS15}, FCN sees the entire image so it implicitly captures the contextual information about the junctions. 
Similar to~\cite{RedmonDGF16, RedmonF16}, our network divides the input image into an $H\times W$ mesh grid, see Fig.~\ref{fig:model} right. If the center of a junction falls into a grid cell, that cell is responsible for detecting it. Thus, each $ij$-th cell predicts a confidence score $c_{ij}$ reflecting how confident the model thinks there exists a junction in that cell. To further locate the junction, each $ij$-th cell also predicts its relative displacement $\x_{ij}$ w.r.t. the center of the cell. Note that the behavior of the grid cells resembles the so-called ``anchors'', which serve as regression references in the latest object detection pipelines~\cite{RenHGS15, RedmonDGF16, Liu2016SSD}.

\noindent{\bf Multi-bin representation for junction branches.} Unlike traditional object detection tasks, each cell in our network needs to make different numbers of predictions due to the varying number of branches in a junction. To address this issue, we borrow the idea of spatial grid and propose a new multi-bin representation for the branches, as shown in Fig.~\ref{fig:model} left. We divide the circle (i.e., from 0 to 360 degrees) into $K$ equal bins, with each bin spanning $ \frac{360}{K}$ degrees. Let the center of the $k$-th bin be $b_k$, we then represent an angle $\theta$ as $(k, \Delta_k)$, if $\theta$ fall into the $k$-th bin, where $\Delta_k$ is the angle residual from the center $b_k$ in the clockwise direction. Thus, for each bin we regress to this local orientation $\Delta_k$.

As a result, our network architecture consists of an encoder and two sets of decoders. The encoder takes the whole image as input and produces an $H\times W$ grid of high-level descriptors via a convolutional network. The decoders then use the feature descriptors to make junction predictions.  
Each junction is represented by $\p_{ij} = \big(\x_{ij}, c_{ij}, \{\theta_{ijk}, c_{ijk}^{\theta}\}_{k=1}^K \big)$, where $\x_{ij}$ is the coordinates of the junction center, $c_{ij}\in [0,1]$ is the confidence score for the presence of a junction in the $ij$-th grid cell, $\theta_{ijk}$ is the angle for the branch in the $k$-th bin, and $c_{ijk}$ is the confidence score for the bin. The two sets of decoders predict the junction center and the branches respectively. Each FCN decoder is simply a convolutional layer followed by a regressor, as shown in Fig.~\ref{fig:system} top.

Unlike local junctions, the junctions we aim to detect each is formed by the intersection of two or more long line segments (the branches). While the junction detection does not explicitly rely on edge/line detection as an intermediate step, the knowledge about the associated edges is indirectly learned by enforcing the network to make correct detection of the branches and their directions.

 

% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=0.7\linewidth]{plot/intervals.png}
%     \caption[Representation of direction angle.]{Representation of direction angle.}
%     \label{fig:intervals}
% \end{figure}

\subsubsection{Loss Function}\vspace{-2mm}

%We use part of popular deep network models as our feature extractor, choices include Inception [cite], ResNet [cite].
To guide the learning process towards the desired output, our loss function consists of four modules. Given a set of ground truth junctions $\P = \{\p_1, \ldots, \p_N\}$ in an image, we write the loss function as follows:\vspace{-2mm}
\begin{equation}
L = \lambda_{conf}^c L_{conf}^c +  \lambda_{loc}^c L_{loc}^c +  \lambda_{conf}^b L_{conf}^b  +  \lambda_{loc}^b L_{loc}^b. %  + \lambda_e L_e.
\label{eq:obj}\vspace{-2mm}
\end{equation}
In the following, we explain each term in more detail.

%Above the feature extractor, we build our decoder modules containing: 
%\begin{compactenum}
%     \item Junction confidence decoder, result in a tensor $J_{conf}$ of $H * W * 2$.
%      \item Junction location decoder, result in a tensor  $J_{loc}$ of $H * W * 2$.
%      \item Angle "bin" (interval) confidence decoder. The tensor $B_{conf}$ of shape $H * W * (2  *K )$.
%     \item Angle residual off the "bin" center decoder.  Tensor $B_{res}$ is of shape  $H * W * K $. 
%      \item ([optional]) An edge decoder, $E$ of $H * W$
% \end{compactenum}

\noindent{\bf Junction center confidence loss $L_{conf}^c$.} The junction center confidence decoder predicts a score $\hat{c}_{ij}$, indicating the probability of a junction for each grid cell. Let ${c}_{ij}$ be the ground truth binary class label, we use the cross-entropy loss:
\begin{equation}\label{eq:loss1}
\small
L_{conf}^c = - \frac{1}{H\times W} \sum_{i, j} E(\hat{c}_{ij}, {c}_{ij}).
\end{equation}

\noindent{\bf Junction center location loss $L_{loc}^c$.} The junction center location decoder predicts the relative position $\hat{\x}_{ij}$ of a junction for each grid cell. We compare the prediction with each ground truth junction using the $\ell_2$ loss:\vspace{-2mm}
\begin{equation}
\small
L_{loc}^c = - \frac{1}{N}\sum_{n=1}^N \| \hat{\x}_{f(n)} - \x_{f(n)}\|_2^2,\vspace{-2mm}
\end{equation}
where $f(n)$ returns the index of the grid cell that the $n$-th ground truth junction falls into, and ${\x}_{f(n)}$ is the relative position of the ground truth junction w.r.t. that cell center.

% Note that, in our actual experiment, among the $H*W$ image grids, most are without junction. So $G_{loc}$ is sparse. Averaging over all grids will result in small loss, which is not expected. Usually, we average over all valid junction in ground-truth.

\noindent{\bf Junction branch confidence loss $L_{conf}^b$.} The junction branch confidence decoder predicts a score $\hat{c}_{ijk}^{\theta}$ for each bin in each grid cell, indicating the probability of a junction branch in that bin. Similar to the junction center confidence loss above, we use the cross-entropy loss to compare the predictions with the ground truth labels. The only difference is that we only consider those grid cells in which a ground truth junction is present:\vspace{-2mm}
\begin{equation}\label{eq:loss2}
\small
L_{conf}^{b} = - \frac{1}{N\times K} \sum_{n=1}^N \sum_{k=1}^K E(\hat{c}_{f(n),k}^{\theta}, {c}_{f(n),k}^{\theta}).\vspace{-2mm}
\end{equation}
   
\noindent{\bf Junction branch location loss $L_{loc}^b$.} Similar to the junction center location loss, we first decide, for each ground truth junction, the indices of the bins that its branches fall into, denoted as $g(r), r=1, \ldots, R_n$, where $R_n$ is the order of $\p_n$. Then, we compare our predictions with the ground truth using the $\ell_2$ loss:\vspace{-2mm}
\begin{small}
\begin{equation}
L_{loc}^b  = - \frac{1}{N}\sum_{n=1}^N \big( \frac{1}{R_n}\sum_{r=1}^{R_n} \|\hat{\theta}_{f(n), g(r)} - {\theta}_{f(n), g(r)}\|_2^2  \big).\vspace{-2mm}
\end{equation}
\end{small}

%\medskip
%\noindent{\bf Edge detection loss $L_e$.} Apart from the above loss functions for the specific targets, we also include a loss for the auxiliary edge detection task. Specifically, our edge decoder predicts a score $e_{ij}$, indicating the probability of being an edge pixel. Following the design in the recent edge detection method HED~\cite{XieT15}, we employ a class-balanced variation of the cross-entropy loss for edge regression:
%\begin{equation}
%L_e  = \frac{1}{H\times W}\sum_{i,j} w^{+} {e}_{ij}  \log(\hat{e}_{ij}) + w^{-} (1 - {e}_{ij}) \log(1- \hat{e}_{ij}),
%\label{eq:edge}
%\end{equation}
%where $w^+$ and $w^-$ are the weights for positive and negative samples, respectively, and ${e}_{ij} \in \{0, 1\}$ is the ground-truth edge class cell for the $(i,j)$-th grid cell. 


\noindent{\bf Implementation details.} We construct our model to encode an image into $60\times 60$ grid of 256-dimensional features. Each cell in the grid is responsible for predicting if a junction is present in the corresponding image region. Our encoder is based on Google's Inception-v2 model~\cite{Szegedy2016RethinkingTI}, which extracts multi-scale features and is well-suited for our problem. For our problem, we only use the early layers in the Inception network, i.e., the first layer to ``Mixed\_3b''. Each decoder consists of a $3\times3\times256$ convolutional layer, followed by a ReLU layer and a regressor. Note that the regressor is conveniently implemented as $1\times1\times d$ convolutional layer, where $d$ is the dimension of the output.

Our network is trained from scratch using the open source framework Tensorflow. The default values for the weights in Eq.~\eqref{eq:obj} are set to the following: $\lambda_{conf}^c = \lambda_{conf}^b = 1, \lambda_{loc}^c=\lambda_{loc}^b=0.1$. We choose the number of bins $K=15$. During training, we adopt the Stochastic Gradient Descent (SGD) method. The momentum parameter is set to 0.9, and the batch size is set to 1. We follow the standard practice in training deep neural networks to augment the data with image domain operations including mirroring, flipping upside-down, and cropping. The initial learning rate is set to 0.01. We decrease the learning rate by a multiple of 0.1 every 100,000 iterations. Convergence is reached at 300,000 iterations.

%\medskip
%\noindent{\bf Balancing positive and negative samples.} Junctions appear in an image at various scales, and the distribution of their locations is often highly uneven. Recall that our method casts junction detection as a binary classification problem for each grid cell, assuming that there is at most one junction in each grid cell. Therefore, we need to use a fairly dense mesh grid (e.g., $60\times 60$) in order to detect junctions with small scales. As a result, only a very small portion of the grid cells contain a junction, leading to an imbalanced positive and negative sample sizes. 

%To mitigate this class imbalance problem, we propose to sample negative grid cells in an image at each iteration, so that the ratio between the number of negative samples and positive samples does not exceed certain threshold $r_{\max}$. By default, we set $r_{\max}=7$ in this paper. 

%%In addition, for the auxiliary edge detection task, we adopt a simple re-weighting strategy to balance the loss between the positive and negative classes as shown in Eq.~\eqref{eq:edge}, where $w^+ = |E^+| / |E|$ and $w^- = |E^-| / |E|$. $|E^+|$ and $|E^-|$ denote the edge and non-edge ground truth label sets, respectively. Note that the same strategy is also utilized in the recent edge detection work~\cite{XieT15}.

\subsection{Line Detection}
Next we design and train a convolutional neural network (Fig.~\ref{fig:system} bottom) to infer line information from RGB images. The network predicts for each pixel $p$ whether it falls on a (long) line $\l$. To suppress local edges, short lines, and curves, the predicted value $h(p)$ (of the heat map) at pixel $p$ is set to be the length of the line it belongs to. Given an image with ground truth lines $\L$, the target value for $h(p)$ is defined to be:\vspace{-2mm}
\begin{equation}
    h(p) = 
    \begin{cases} 
        d(\l)     &   \text{$p$ is on a line $\l$ in $\L$}, \\
        0       &   \text{$p$ is not on any line in $\L$}, 
    \end{cases} \vspace{-2mm}
\end{equation}
where $d(\l)$ is the length of the line $\l$. Let $\hat{h}(p)$ be the estimated heatmap value, then the loss function we try to minimize the $\ell_2$ loss:\vspace{-2mm}
\begin{equation}
L = \sum_{i,j} \| \hat{h}(p_{ij}) - h(p_{ij})\|^2_2.\vspace{-2mm}
\end{equation}
where the sum is over all pixels of the image. 

\noindent{\bf Implementation details.}  The network architecture is inspired by the Stacked Hourglass network~\cite{NewellYD16}. It takes a $256 \times 256$ RGB image as input, extracts a $64 \times 64 \times 256$ feature maps via two Pyramid Residual Modules (PRM), see Fig. \ref{fig:system} bottom. The feature maps then go through five stacked hourglass modules, followed by two fully convolutional and ReLU layers ($5\times 5\times 32$ and $5\times 5\times 16$) and a $5 \times 5 \times 1$ convolutional layer  to output a $256 \times 256$ pixel-wise heat map. The detailed pyramid residual module and stacked hourglass module can be found in ~\cite{NewellYD16}.

During training, we adopt the Stochastic Gradient Descent (SGD) method. The momentum parameter is set to 0.9, and the batch size is set to 4. Again, we augment the data with image domain operations including mirroring, flipping upside-down. The initial learning rate is set to 0.001. Convergence is reached at 150,000 iterations.

Notice that we have used an Inception network for junction detection whereas an hourglass network for line detection. In junction detection, we are not interested in the entire support of the line, hence the receptive field of an Inception network is adequate for such tasks. However, we find that for accurately detecting lines with large spatial support, the Stacked Hourglass network works much better due to its large (effective) receptive field. In addition, our experiment also shows that above length-dependent $\ell_2$ loss is more effective than the cross-entropy cost often used in learning-based edge detection.  


\subsection{Combine Junctions and Lines for Wireframe}
The final step of the system is to combine the results from junction detection and line detection to generate a wireframe $\W$ for the image, which, as mentioned before, consists of a set of junction points $\P$ connected by a set of line segments $\L$. 

We determine the set of junctions and line segments connecting them based on the following rules and procedure:\vspace{-1mm}
%\begin{enumerate}
%\item The set $\P$ is initialized with the output from the junction detector. A pair of detected junctions $\p$ and $\mathbf{q} \in \P$ are connected by a line segment $\l = (\p, \mathbf{q})$ if they are on (or close to be on) each other's branches, and we add this segment $\l$ to $\L$. If there are multiple detected junctions on the same branch of a junction point $\p$, we only keep the shortest segment to avoid overlap.\footnote{Hence we are less interested in detecting a straight line with the longest possible support, instead, we are interested in its incidence relationship with other lines and junctions.} \vspace{-1mm}
%\item For any branch of a junction $\p$ that is not connected to any other junction, if the support of the detected line heat map $h$ aligns well with the branch, we then connect the junction to the furthest end point $\mathbf{q}$ of the line support. If this new segment $\l = (\p, \mathbf{q})$ intersects with any prior line segments in $\L$, we add the intersections to $\P$ and all the intermediate segments to $\L$.
%\end{enumerate}
\begin{itemize}
	\item[1.] Our algorithm starts from the output of the junction detector, \ie a set of junctions $\{ \p_{i}\}_{i = 1}^N$, $\p_{i} = \big(\x_{i}, \{\theta_{ik}\}_{k=1}^{K_i} \big)$. Each branch $\theta_{ik}$ results in a ray $r_{ik}$ starting from $p_i$. We collect all the possible rays. Then we check each pair of rays starting from different junctions whether they are opposite on the same line segment. If ray $r_{ik}$ is opposite of $r_{jt}$ then $p_i$ and $p_j$ are candidate opposite for each other, \ie there might be a line segment between $p_i$ and $p_j$. When a ray with multiple matches, we only keep the shortest line segment to avoid overlap.  
	\item[2.]
\end{itemize}

Notice that both the sets $\P$ and $\L$ may have {\em two} sources of candidates. For the junction set $\P$, besides those directly detected by the junction detection, the line segments could also produce new intersections or endpoints that were missed by the junction detection. For the line segment set $\L$,  it could come from branches of the detected junctions and the line detection. 

We leave more detailed description of the algorithm to the supplementary material. Of course, there could be more advanced ways to merge the detected junctions and line heat map which we will explore in future work. Nevertheless, from our experiments (see next section), we find that the results from junction detection and line detection are rather complementary to each other and the above simple procedure already produces rather decent results. 


 



==> 5experiment-kun.tex <==
% !TEX root = cvpr18-parsing.tex
\section{Experiments}

In this section, we conduct extensive experiments to evaluate the quality of junctions and final wireframes generated by our method, and compare it to the state-of-the-art. All experiments are conducted on one NVIDIA Titan X GPU device. In testing phase, our method runs at about two frames per second, thus our method is potentially suitable for applications which require real-time processing.

\subsection{Datasets and Evaluation Metrics}

For performance evaluation, we split our wireframe dataset into a training set and a testing set. Among the 5,462 images in the dataset, 5,000 images are randomly selected for training and validation, and the remaining 462 images are used for testing. For junction detection (Section~\ref{sec:exp:junction}), we compare the junctions detected by any method with the ground truth junctions (Fig.~\ref{fig:data}, second row). For wireframe construction (Section~\ref{sec:exp:wireframe}), we compare the line segments detected by any method with the ground truth line segments labeled by human subjects (Fig.~\ref{fig:data}, first row).

For both junction detection and wireframe construction experiments, all methods are the evaluated quantitatively by means of the \emph{recall} and \emph{precision} as described in~\cite{MartinFM04, MaireAFM08, XiaDG14}. In the context of junction detection, recall is the fraction of true junctions that are detected, whereas precision is the fraction of junction detections that are indeed true positives. In the context of wireframe construction, recall is the fraction of line segment pixels that are detected, whereas precision is the fraction of line segment pixels that are indeed true positives.

Specifically, let $G$ denote the set of ground truth junctions (or line segment pixels), and $Q$ denote the set of junctions (or line segment pixels) detected by any method, the precision and recall are defined as follows:\vspace{-2mm}
\begin{equation}
\mbox{Precision} \doteq {\left| G\cap Q\right|}/{\left| Q \right|}, \;\; \mbox{Recall} \doteq {\left| G\cap Q\right|}/{\left| G \right|}.\vspace{-2mm}
\end{equation}
Note that, following the protocols of previous work~\cite{MartinFM04, MaireAFM08, XiaDG14},  the particular measures of recall and precision allow for some small tolerance in the localization of the junctions (or line segment pixels). In this paper, we set the tolerance to be 0.01 of the image diagonal.


%We evaluate our performance via two metrics, i.e., precision and recall. Specifically, for junction location quantification, we refer to the evaluation method for edge detection in \cite{Dollr2013StructuredFF}. In testing phase, we fix a distance threshold, and assigning prediction to ground-truth junction locations accordingly within threshold, and we compute the precision and recall after assignment. The precision measures how accurately junction detector is. In some cases, algorithm with high recall fall into low precision for detecting too many redundant junction, while some detectors reporting high accuracy actually detect only little part of junctions. So these two metric is well-suited for junction detection task.

\subsection{Junction Detection Comparison}
\label{sec:exp:junction}
We compare our junction detection method with two recent methods \footnote{Details about these methods are in supplementary material.}, namely Manhattan junction detection (MJ)~\cite{RamalingamPJT13} and \emph{a contrario} junction detection (ACJ)~\cite{XiaDG14}.

%\noindent{\bf MJ~\cite{RamalingamPJT13}}: This method detects Manhattan junctions formed by line segments in three principal orthogonal directions using a simple voting-based scheme. %Specifically, let $vp_x$, $vp_y$, and $vp_z$ be the vanishing points associated with the three principal directions, it build six accumulators that store votes $V_j$, where $j\in \{ x^+. x^-, y^+, y^-, z^+, z^-\}$, for a subset of points uniformly sampled from the original image. For each point $p$, every line segment that is collinear with the line joining $p$ and $vp_i, i\in \{x,y,z\}$, votes for either $V_{i^+}(p)$ or $V_{i^-}(p)$ depending on its location with respect to $p$ and $vp_i$. Finally, different types of junctions are detected by applying a product operation to the contents of the six accumulators.
%As the authors did not release their code, we use our own implementation of the method. Line segments are first detected using LSD~\cite{von2012lsd}, and then clustered using J-Linkage~\cite{Tardif09} to obtain the vanishing points. Note that this method only applies to scenes that satisfy the Manhattan world assumption. For fair comparison, we only keep the images in which three principal vanishing points are detected. An important parameter in our implementation is the maximum distance $d_{\max}$ between a line segment and a point $p$ for that line segment to vote for $p$. We vary the value $d_{\max} \in \{10, 20, 30, 50, 100, 200, 300, 500\}$ pixels.
%
%\noindent{\bf ACJ~\cite{XiaDG14}}: This method relies on statistical modeling of image gradients and an \emph{a contrario} approach to detect junctions. Specifically, meaningful junctions are detected as those which are very unlikely under a null hypothesis $\mathcal{H}_0$, which is defined based on the distribution of gradients of arbitrary natural images. In the method, each candidate junction is associated with a strength value depending on the image gradients around it. Then, the candidate junction is validated with a threshold, which is derived by controlling the number of false detections, $\epsilon$, in an image following $\mathcal{H}_0$. For the experiments, we use the implementation provided by the authors of~\cite{XiaDG14} and vary the value $\epsilon \in \{10^{-3}, 10^{-2}, 10^{-1}, 1, 10^1, 10^2, 10^3\}$.


\begin{figure}[t]
    \centering
    \includegraphics[width = 1.7in]{plot/pr.pdf}
    \caption{The precision-recall curves of different junction detection methods on our test dataset.\vspace{-3mm}}
    \label{fig:pr}
\end{figure}

\noindent{\bf Performance comparison.} Fig.~\ref{fig:pr} shows the precision-recall curves of all methods on our new dataset. For our method, we compute the precision-recall curve by varying the junction confidence threshold $\tau$ from 0.1 to 0.9. As one can see, our method outperforms the other methods by a large margin. Fig.~\ref{fig:results} compares qualitatively the results of all methods on our test data. Compared to the other two methods, MJ tends to miss important junctions due to the imperfect line segment detection results. Moreover, since MJ relies on local image features, it noticeably produces quite a few repetitive detections around some junctions. By directly modeling the image gradients, ACJ is able to find most junctions on the scene structures. However, as a local method, ACJ makes a lot of false predictions on textured regions (e.g., floor of the first, sky of the fourth image). In contrast, our method is able to detect most junctions intersected by salient lines, while minimizing the number of false detections. This is no surprise because our supervised framework implicitly encodes high-level structural and semantic information of the scene as it learns from the labeled data provided by humans.


\subsection{Line Segment Detection Comparison}
\label{sec:exp:wireframe}
In this section, we compare the wireframe results of our method with two state-of-the-art line segment detection methods \footnote{Details about these methods are in supplementary material.}, namely the Line Segment Detector (LSD) ~\cite{von2012lsd} and the Markov Chain Marginal Line Segment Detector (MCMLSD)~\cite{Almazan17}. We test and compare with these methods on both our new dataset and the York Urban dataset \cite{Denis2008EfficientEM} used in the work of MCMLSD \cite{Almazan17}.

%\noindent{\bf LSD~\cite{von2012lsd}}: This method is a linear-time line segment detector that requires no parameter tuning. The algorithm includes three stages. The first stage grows regions from pixels as line support; and the second stage approximates the line segment with a rectangle; finally, a potential line segment is validated as true detection if it satisfies a threshold criterion based on its length and the number of points aligned. For the comparison here, we use the code released by the authors.\footnote{http://www.ipol.im/pub/art/2012/gjmr-lsd/}  To generate the precision and recall curve, similar to \cite{von2012lsd}, we set thresholds for $-\log$(NFA) (NFA is the number of false alarms) from $0.01*\{1.75^0, 1.75^1, 1.75^2, ..., 1.75^{19}\}$.
%
%
%\noindent{\bf MCMLSD~\cite{Almazan17}}: This method proposes a two-stage algorithm for finding line segments. At the first stage, they employ the probabilistic Hough transform to identify globally optimal lines. In the second stage, they search each of these lines for their supports (segments) in the image. The search for segments from 2D images is simplified to finding 1D segments along a long line, which allows the problem to be modeled as labeling hidden states in a linear Markov chain model. In the comparison, we use the code released by the authors.\footnote{http://www.elderlab.yorku.ca/resources/} Be aware that authors of \cite{Almazan17} have introduced a different metric than ours that tends to penalize over-segmentation. Hence our metric can be unfair to their method. Nevertheless, our metric is more appropriate for wireframe detection as we prefer to interpret a long line as several segments between junctions if it intersects with other lines.

\begin{figure}[t]
    \centering
    \includegraphics[width = 1.62in]{plot/LinePR_ours.pdf}
    \includegraphics[width = 1.62in]{plot/LinePR_york.pdf}
    \caption{The precision-recall curves of different line segment detection methods. {\bf Left:} on our test dataset. {\bf Right:} on the York Urban dataset \cite{Denis2008EfficientEM}. \vspace{-3mm}}
    \label{fig:LinePR-ours} \label{fig:LinePR-york}
\end{figure}

\begin{figure*}[t!]
\centering
%\includegraphics[height =1.2in]{plot/draw.pdf} &

\includegraphics[height=0.9in]{plot/results/00066618-cvpr13.jpg}
\includegraphics[height=0.9in]{plot/results/00072768-cvpr13.jpg}
\includegraphics[height=0.9in]{plot/results/00036977-cvpr13.jpg}
\includegraphics[height=0.9in]{plot/results/00076835-cvpr13.jpg}
\includegraphics[height=0.9in]{plot/results/00194897-cvpr13.jpg}
\\
\includegraphics[height=0.9in]{plot/results/00066618-acj.jpg}
\includegraphics[height=0.9in]{plot/results/00072768-acj.jpg}
\includegraphics[height=0.9in]{plot/results/00036977-acj.jpg}
\includegraphics[height=0.9in]{plot/results/00076835-acj.jpg}
\includegraphics[height=0.9in]{plot/results/00194897-acj.jpg}
\\
\includegraphics[height=0.9in]{plot/results/00066618-binNet.jpg}
\includegraphics[height=0.9in]{plot/results/00072768-binNet.jpg}
\includegraphics[height=0.9in]{plot/results/00036977-binNet.jpg}
\includegraphics[height=0.9in]{plot/results/00076835-binNet.jpg}
\includegraphics[height=0.9in]{plot/results/00194897-binNet.jpg}
\\
\caption{Junction detection results. {\bf First row:} MJ ($d_{\max}=20$). {\bf Second row:} ACJ ($\epsilon=1$). {\bf Third row:} Our method ($\tau=0.5$). }
\label{fig:results}
\end{figure*}


\nop{
\begin{figure*}[t]
\centering
\includegraphics[width =6.2in]{plot/LineComp.png}
\caption{Line/wireframe detection results. {\bf First row:} LSD (-$\log$(NFA) > $0.01*1.75^8$). {\bf Second row:} MCMLSD (confidence top 100). {\bf Third row:} Our method (line heat map $h(p)> 10$). {\bf Fourth row:} Ground truth.}
\label{fig:line-results}
\end{figure*}
}

\begin{figure*}[t!]
\centering
\includegraphics[height=0.88in]{plot/fig8/00031608_lsd.jpg}
\includegraphics[height=0.88in]{plot/fig8/00036242_lsd.jpg}
\includegraphics[height=0.88in]{plot/fig8/00055416_lsd.jpg}
\includegraphics[height=0.88in]{plot/fig8/00064984_lsd.jpg}
\includegraphics[height=0.88in]{plot/fig8/00075103_lsd.jpg}
\\
\includegraphics[height=0.88in]{plot/fig8/00031608_mcm.jpg}
\includegraphics[height=0.88in]{plot/fig8/00036242_mcm.jpg}
\includegraphics[height=0.88in]{plot/fig8/00055416_mcm.jpg}
\includegraphics[height=0.88in]{plot/fig8/00064984_mcm.jpg}
\includegraphics[height=0.88in]{plot/fig8/00075103_mcm.jpg}
\\
\includegraphics[height=0.88in]{plot/fig8/00031608_4.jpg}
\includegraphics[height=0.88in]{plot/fig8/00036242_4.jpg}
\includegraphics[height=0.88in]{plot/fig8/00055416_4.jpg}
\includegraphics[height=0.88in]{plot/fig8/00064984_4.jpg}
\includegraphics[height=0.88in]{plot/fig8/00075103_4.jpg}
\\
\includegraphics[height=0.88in]{plot/fig8/00031608_gt.jpg}
\includegraphics[height=0.88in]{plot/fig8/00036242_gt.jpg}
\includegraphics[height=0.88in]{plot/fig8/00055416_gt.jpg}
\includegraphics[height=0.88in]{plot/fig8/00064984_gt.jpg}
\includegraphics[height=0.88in]{plot/fig8/00075103_gt.jpg}
\\
\caption{Line/wireframe detection results. {\bf First row:} LSD (-$\log$(NFA)  $> 0.01*1.75^8$). {\bf Second row:} MCMLSD (confidence top 100). {\bf Third row:} Our method (line heat map $h(p) > 10$). {\bf Fourth row:} Ground truth.}\vspace{-2mm}
\label{fig:line-results}
\end{figure*}


\noindent{\bf Performance comparison.} Fig.~\ref{fig:LinePR-ours} shows the precision-recall curves of all methods on our dataset and the York Urban dataset, respectively. As one can see, our method outperforms the other methods by a significant margin on our dataset. The margin on the York Urban dataset is decent but not so large. According to \cite{Almazan17}, the labeling of the York Urban dataset is not as complete for salient line segments, hence it is not entirely suitable for the wireframe detection task here.  Fig.~\ref{fig:line-results} compares qualitatively the results of all methods on our test data. Since the other two methods rely on local measurements, they tend to produce many line segments on textured regions (e.g. curtain of the first image) which do not correspond to scene structures.

